Cross-language Learning with Adversarial Neural Networks: Application to Community Question Answering

We address the problem of cross-language adaptation for question-question similarity reranking in community question answering, with the objective to port a system trained on one input language to another input language given labeled training data for the first language and only unlabeled data for the second language. In particular, we propose to use adversarial training of neural networks to learn high-level features that are discriminative for the main learning task, and at the same time are invariant across the input languages. The evaluation results show sizable improvements for our cross-language adversarial neural network (CLANN) model over a strong non-adversarial system.

==> model.tex <==
We demonstrate our approach for cross-language representation learning with adversarial training on a cross-lingual extension of the \emph{question--question similarity reranking} subtask of SemEval-2016 Task~3 on community Question Answering \cite{nakov-EtAl:2016:SemEval}.

An example %for the original monolingual 
for the monolingual task is shown in Figure~\ref{fig:example}. We can see an English input original question $q$ and a list of several potentially similar questions $q_i^{\prime}$ from the Qatar Living\footnote{http://www.qatarliving.com/forum} forum, retrieved by a search engine. The original question (also referred to as a new question) asks about how to tip in Qatar. Question $q_1^{\prime}$ is relevant with respect to it as it asks the same thing, and so is  $q_2^{\prime}$, which asks how much one should tip in a specific situation. However, $q_9^{\prime}$ and $q_{10}^{\prime}$ are irrelevant: the former asks about what to wear at business meetings, and the latter asks about how to tip a kind of person who does not normally receive tips.

%\setarab
%\resizebox{\textwidth}{!}{\begin{tabular}{p{10cm}}<'`.tA' Albq^sy^s? hl tqwmwn b_dlk; '_dA kAnt Al'^gAbT bn`m, fmA mqdAr mA ttrkwnh? fy blAdnA, ntrk 15 - 20 bAlmA'T.>\end{tabular}}


In our case, the input question $q$ is in a different language (Arabic) than the language of the retrieved questions (English).
The goal is to rerank a set of $K$ retrieved questions $\{q'_{k}\}_{k=1}^{K}$ written in a source language (e.g., English) according to their similarity with respect to an input user question $q$ that comes in another (target) language, e.g.,~Arabic. For simplicity, henceforth we will use Arabic as target and English as source. However, in principle, our method generalizes to any source-target language pair.


%\subsection{Unsupervised Model}
\subsection{Unsupervised Language Adaptation}

We approach the problem as a classification task, where given a 
%new question-related 
question pair $(q, q')$, the goal is to decide whether $q'$ is \emph{similar} to $q$ or not. Let $c\in\{0,1\}$ denote the class label -- \blue{1 for similar and 0 for not similar}. We use the posterior probability $p(c = 1|q,q',\theta)$ as a score for ranking, where $\theta$ represents the model parameters.

\blue{Let $\Rs_n = \{q'_{n,k}\}_{k=1}^{K}$ denote the set of $K$ retrieved questions for a new question $q_n$. Note that the questions in $\Rs_n$ are always in English. We consider a training scenario where we have labeled examples $\Ds_S = \{q_n, q'_{n,k}, c_{n,k} \}_{n=1}^{N}$ for English $q_n$, and unlabled examples $\Ds_T = \{q_n, q'_{n,k}\}_{n=N+1}^{M}$ for Arabic $q_n$ \blue{with $c_{n,k}$ denoting the class label for the pair $(q_n, q'_{n,k})$}. We aim to train a cross-language model that can classify any test example $\{q_n,  q'_{n,k}\}$,} where $q_n$ is in Arabic. This scenario is of practical importance, for instance when an Arabic speaker wants to query the system in Arabic, %for a particular question, 
and the database of related information is only in English. 
We use the adversarial training of neural networks for domain adaptation proposed by \newcite{Ganin:2016:DTN:2946645.2946704}. %(\emph{Domain-adversarial Neural Networks}, or DANN).

\begin{figure*}[t]
\centering
\hspace*{-1mm}\includegraphics[width=0.65\linewidth]{figures/CLANN-final}\caption{\label{f-clann} Architecture of CLANN for the question to question similarity problem in cQA.}
%\vspace{-4mm}
\end{figure*}


Figure \ref{f-clann} shows the architecture of our cross-language adversarial neural network (CLANN) model. The input to the network is a pair $(q, q')$, which is first mapped to fixed-length vectors $(\mathbf{z}_{q}, \mathbf{z}_{q'})$. We can use existing tools like word2vec \cite{Mikolov:2013} trained on the respective languages to get these embeddings. Alternatively, we can use cross-language representation learning methods like bivec \cite{luong-pham-manning:2015:VSM-NLP}. The cross-language embeddings can give the network better initializations, and can be crucial when the labeled set is too small to train the input representations directly with the end-to-end system.

The network then models the interactions between the input embeddings by passing them through two non-linear hidden layers, $\mathbf{h}$ and $\mathbf{f}$.  Additionally, the network considers \emph{pairwise} features $\phi(q,q')$ that go directly to the output layer, and also through the second hidden layer. 

The following equations describe the transformations through the hidden layers: 

\begin{eqnarray}
\mathbf{h} &=&  g(U [\mathbf{z}_{q};\mathbf{z}_{q'}]) \\
\mathbf{f} &=&  g(V [\mathbf{h};\phi(q, q')]) \label{eq:f}
\end{eqnarray}

%$\mathbf{h} =  g(U [\mathbf{z}_{q},\mathbf{z}_{q'}])$; $\mathbf{f} =  g(V [\mathbf{h},\phi(q, q')])$ 
%\smallskip 

\noindent where \blue{$[.;.]$ denotes concatenation of two column vectors,} $U$ and $V$ are the weight matrices in the first and in the second hidden layer, and $g$ is a nonlinear activation function; we use rectified linear units or ReLU \cite{icml2010_NairH10}.  

\blue{The pairwise features $\phi(q,q')$ encode different types of similarity between $q$ and $q'$, and task-specific properties as we describe them later in Section~\ref{sec:setting}. In our earlier work \cite{Giovanni2017_sigir}, we found it beneficial to use them directly to the output layer as well as through a hidden-layer transformation. The non-linear transformation allows us to learn high-level abstract features from the raw similarity measures, while the adversarial training as we describe below will make these abstract features language invariant.} 

%In our adversarial setting, this allows us to learn features that are language invariant.}

% Using them directly gives the advantage of a linear classifier, and can guide learning of other abstract features, }has   while  } 






The classification (output) layer computes a sigmoid: 

\begin{eqnarray}
\hat{c}_{\theta} = p(c = 1|\mathbf{f}, \mathbf{w}) =  \sigm (\mathbf{w}^T [\mathbf{f};\phi(q, q')])
\end{eqnarray}

%$\hat{c}_{\theta} = p(c = 1|\mathbf{f}, \mathbf{w}) =  \sigm (\mathbf{w}^T [\mathbf{f},\phi(q, q')])$, 

\noindent where $\mathbf{w}$ are the output layer weights. 

We learn the network by minimizing the negative log-probability of the gold labels: 

%$\Ls_c(\theta) =  - c_n \log \hat{c}_{\theta} - (1-c) \log \left(1- \hat{c}_{\theta} \right)$.

\begin{eqnarray}
\Ls_c(\theta) =  - c \log \hat{c}_{\theta} - (1-c) \log \left(1- \hat{c}_{\theta} \right)
\end{eqnarray}


The network described so far learns the abstract features through multiple hidden layers that are discriminative for the classification task (\emph{similar} vs. \emph{non similar}). However, our goal is also to make these features invariant across languages. To this end, we put a language discriminator, another neural network that takes the internal representation of the network $\mathbf{f}$ (see Equation \ref{eq:f}) as input, and tries to discriminate between \emph{English} and \emph{Arabic} inputs --- in our case, whether the input is from $\Ds_S$ or from $\Ds_T$. 

The language discriminator is again defined by a sigmoid: 

 
\begin{eqnarray}
\hat{l}_{\omega} = p(l = 1|\mathbf{f}, \omega) = \sigm (\mathbf{w}_l^T \mathbf{h}_l)
\end{eqnarray}


%$\hat{l}_{\omega} = p(l = 1|\mathbf{f}, \omega) = \sigm (\mathbf{w}_l^T \mathbf{h}_l)$, 

\noindent where $l\in\{0,1\}$ denotes the language of $q$, $\mathbf{w}_l$ are the final layer weights of the discriminator, and $\mathbf{h}_l = g(U_l \mathbf{f})$ defines the hidden layer of the discriminator with $U_l$ being the layer weights and $g$ being the ReLU activations. 

We use the negative log-probability as the discrimination loss: 

\begin{eqnarray}
\Ls_l(\omega) =  - l \log \hat{l}_{\omega} - (1-l) \log \left(1- \hat{l}_{\omega} \right) \label{eq:dis-loss}
\end{eqnarray}


\blue{The overall training objective of the composite model can be written as}

%We can write the overall training objective as 

\small
\begin{eqnarray}
\Ls(\theta,\omega) =  
\sum_{n=1}^N \Ls_c^n (\theta) - 
\lambda \Big[ \sum_{n=1}^N \Ls_l^n(\omega) + \sum_{n=N+1}^M \Ls_l^n(\omega) \Big]  \label{loss}
\end{eqnarray}
\normalsize

\noindent where $\theta = \{U,V,\mathbf{w}\}$, $\omega = \{U,V,\mathbf{w},U_l,\mathbf{w}_l\}$, and the hyper-parameter $\lambda$ controls the relative strength of the two networks. 

In training, we seek parameters such that 

\begin{eqnarray}
\theta^* = \argmin_{U,V,\mathbf{w}} \max_{U_l,\mathbf{w}_l} \Ls (U,V,\mathbf{w}, U_l,\mathbf{w}_l) 
\end{eqnarray}

\noindent which involves a maximization \blue{(gradient ascent)} with respect to $\{U_l,\mathbf{w}_l\}$ and a minimization \blue{(gradient descent)} with respect to $\{U,V,\mathbf{w}\}$. \blue{Notice that the maximization  of $\Ls (U,V,\mathbf{w}, U_l,\mathbf{w}_l) $ with respect to $\{U_l,\mathbf{w}_l\}$ is equivalent to minimizing the discriminator loss $\Ls_l(\omega)$ in Equation \ref{eq:dis-loss}, thus is to improve the discrimination accuracy.}  In other words, \blue{when put together,} the updates of the shared parameters $\{U,V,\mathbf{w}\}$ for the two classifiers work adversarially to each other. 

In our gradient descent training, \blue{the min-max optimization} is achieved by reversing the gradients of the language discrimination loss $\Ls_l(\omega)$, when they are backpropagated to the shared layers; \blue{as shown in Figure \ref{f-clann}, the gradient reversal is applied to layer $\mathbf{f}$ and its previous layers. This is related to the training method of Generative Adversarial Networks or GANs \cite{Goodfellow_14_GAN}, where the goal is to build deep generative models that can generate real-like images. The discriminator in GANs tries to separate a real image from a model-generated image, thus the training attempts to minimize the discrepancy between the two distributions (i.e., real vs. model). When backpropagating to the generator network, they consider a slight variation of the reverse gradients with respect to the discriminator loss.\footnote{If $\rho$ is the discriminator probability, instead of reversing the gradients of $\log (1- \rho)$, they use the gradients of $\log \rho$.}} %

   

% where the objective is to generate  





%Moreover, the authors mention the problem of saturating sigmoids which may arise at the
%early stages of training due to the significant dissimilarity of the domains. The technique
%they use to circumvent this issue (the “adversarial” part of the gradient is replaced by a
%gradient computed with respect to a suitable cost) is directly applicable to our method.




\paragraph{Training.}

\blue{Algorithm \ref{alg:training} illustrates the SGD-based algorithm to train our model. We first initialize the model parameters.} We form each minibatch of size $b$ by randomly sampling ${b}/{2}$ labeled examples from $\Ds_S$ and ${b}/{2}$ unlabeled examples from $\Ds_T$. For the labeled instances, both $\Ls_c(\theta)$ and  $\Ls_l(\omega)$ losses are active, while only $\Ls_l(\omega)$ loss is active for the unlabeled instances. 

\small
%\setlength{\textfloatsep}{0.15in}
%\scalebox{0.75}{
\begin{algorithm}[t!]
%\scriptsize
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
%\SetAlgoLined
\SetAlgoNoLine
\SetNlSkip{0em}
\Input{data $\Ds_S$, $\Ds_T$, batch size $b$}
\Output{learned model parameters  $\{U,V,\mathbf{w}, U_l, \mathbf{w}_l \} $}
1. Initialize model parameters; \\
%	\hspace{0.5cm} a. $\psi_c$ for $\Lb_c (\mathbf{v}_i)$ \tcp*{over words}
%    \hspace{0.5cm} b. $\psi_g$ for $\Lb_g (\mathbf{v}_i, \Ns(\mathbf{v}_i))$ \tcp*{over nodes}
2. \Repeat {convergence}{ 
        
		\hspace{-0.1cm} \Na Sample $\frac{b}{2}$ labeled examples from $\Ds_S$ \\
		\hspace{-0.1cm} \Nb Sample $\frac{b}{2}$ unlabeled examples from $\Ds_T$ \\
		\hspace{-0.1cm} \Nc Compute $\Ls_c(\theta)$ and $\Ls_l(\omega)$ \\
		\hspace{-0.1cm} \Nd Take a gradient step for $\frac{2}{b} \nabla_{\theta} \Ls_c(\theta) $  \\
		\hspace{-0.1cm} \Ne Take a gradient step for $\frac{2\lambda}{b} \nabla_{U_l,\mathbf{w}_l} \Ls_l(\omega)$  \\
		\tcp{Gradient reversal}
		\hspace{-0.1cm} \Nf Take a gradient step for $- \frac{2\lambda}{b} \nabla_{\theta} \Ls_l(\omega) $  \\

%        \For{each batch sampled from $\Ds_S^l$}{
%		\Na Compute $\Ls_C(\Lambda, \Phi)$	and $\Ls_D(\Lambda, \Psi)$ \\		 \Nb Take gradient steps for $\Ls_C(\Lambda, \Phi)$ and $\Ls_D(\Lambda, \Psi)$; \\
%        }
   }
\caption{Model Training with SGD}
\label{alg:training}
\end{algorithm}
%}

\normalsize

As mentioned before, the main challenge in adversarial training is to balance the two components of the network. If one component becomes smarter than the other, its loss to the shared layer becomes useless, and the training fails to converge \cite{ArjovskyCB17}. Equivalently, if one component becomes weaker, its loss overwhelms that of the other, causing the training to fail. In our experiments, we observed the language discriminator to be weaker than the task classifier. This could be due to the fact that we used cross-language embeddings to represent $q$ and $q'$, which made the language discriminator confused between source and target languages. To balance the two components, we would want the error signals from the discriminator to be fairly weak initially, with full power unleashed only as the classification errors start to dominate. We follow the weighting schedule proposed by \newcite [p. 21]{Ganin:2016:DTN:2946645.2946704}, which initializes $\lambda$ to $0$, and changes it gradually to $1$ as training progresses. I.e., we start with training the task classifier first, and we gradually add the discriminator's loss.   


   
%As for the main issue, that the reconstruction error overwhelms the adversary, I think this is an expected behavior, especially for the regular auto-encoder (which I assume the plot corresponds to). The adversarial loss is directly tied to the latent representation and therefore gives immediate feedback early during training, and is the primary way that the latent representation is shaped. Once training progresses and reconstruction improves, the gradients from the reconstruction error will overwhelm those from the adversary. To put it differently, the adversarial classifier output gives one bit of information about the latent representation whereas reconstructing even a single word gives much more. The balance is hard to set. 

%- anneal the loss functions so that the adversarial loss weighs more later
%- or successively increase the number of optimization steps for the adversary. This would work only if the adversary is sufficiently powerful. 

%The hyper-parameter $\lambda$ is set adaptively as learning  following the suggested schedule by \newcite{Ganin:2016:DTN:2946645.2946704}.

\subsection{Semi-supervised Extension}
\label{subsec:semisup-model}

Above we considered an unsupervised adaptation scenario, where we did not have any labeled instance for the target language, i.e., when the new question $q_n$ is in Arabic. However, our method can be easily generalized to a semi-supervised setting, where we have access to some labeled instances in the target language, $\Ds_{T^*} = \{q_n, \Rs_n, c_n\}_{n=M+1}^{L}$. In this case, each minibatch during training is formed by labeled instances from both $\Ds_S$ and $\Ds_{T^*}$, and unlabeled instances from $\Ds_T$.  

%the adversarial training with gradient reversal 

% $\{U,V,\mathbf{w}\}$ 


%\vspace{-3mm}
%\small
%\begin{eqnarray}
%\theta^* = \argmin_{U,V,\mathbf{w}} \max_{U_l,\mathbf{w}_l} \Ls (U,V,\mathbf{w}, U_l,\mathbf{w}_l) 
%\end{eqnarray}
%\normalsize
%\vspace{-2mm}


%\begin{eqnarray}
%\Ls(U,V,\mathbf{w},U_l,\mathbf{w}_l) = \sum_{n=1}^N \Ls_c^n (U, V, \mathbf{w}) - \nonumber \\ 
%\lambda \Big[ \sum_{n=1}^N \Ls_l^n(U,V,\mathbf{w},U_l,\mathbf{w}_l) + \sum_{n=N+1}^N \Ls_l^n(U,V,\mathbf{w},U_l,\mathbf{w}_l) \Big]  
%\end{eqnarray}



















